Meterwavelength Single-pulse Polarimetric Emission Survey. VI. Towards understanding the Phenomenon of Pulsar Polarization in Partially Screened Vacuum Gap model

We have observed 123 pulsars with periods longer than 0.1 seconds in the Meterwavelength Single-pulse Polarimetric Emission Survey. In this work a detailed study of polarization behaviour of these pulsars have been carried out. We were able to fit the rotating vector model to the polarization position angle sweeps in 68 pulsars, and in 34 pulsars the emission heights could be measured. In all cases the radio emission was constrained to arise below 10\% of the light cylinder radius. In pulsars with low spindown energy loss, $\dot{E}<10^{34}$ ergs s$^{-1}$, we found the mean fractional linear polarization of the individual times samples in single pulses to be around 0.57 (57\%) which is significantly larger than the fractional linear polarization of 0.29 (29\%) obtained from the average profiles. On the other hand the mean fractional circular polarization of the individual time samples in single pulses is around 0.08 (8\%), similar to the measurements from the average profiles. To explain the observed polarization features, we invoke the partially screened vacuum gap model of pulsars, where dense spark associated plasma clouds exist with high pair plasma multiplicity, with significant decrease of density in the regions between the clouds, that are dominated by iron ions. The coherent radio emission is excited by curvature radiation from charge bunches in these dense plasma clouds and escape as linearly polarized waves near cloud boundaries. We suggest that the circular polarization arises due to propagation of waves in the low pair multiplicity, ion dominated inter-cloud regions.

==> figset.tex <==
\figsetstart
\figsetnum{1}
\figsettitle{Single pulse polarization behaviour}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.1}
\figsetgrptitle{PSR J0034-0721}
\figsetplot{J0034-0721_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0034-0721_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{J0034-0721_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J0034-0721_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J0034-0721_602MHz_20Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total 
intensity (Stokes I; solid black lines), total linear polarization (dashed red 
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with 
the average PPA (red error bars). The RVM fits to the average PPA (dashed pink 
line) is also shown in this plot. Middle panel show 
the $\chi^2$ contours only for 333 MHz and the correlated parameters $\alpha$ and $\beta$ obtained from RVM
fits. Bottom panel shows the Hammer-Aitoff projection of the polarized time 
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\figsetgrpstart
\figsetgrpnum{singlpol.2}
\figsetgrptitle{PSR J0151-0635}
\figsetplot{J0151-0635_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0151-0635_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J0151-0635_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0151-0635_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0151-0635_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J0151-0635_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total  
intensity (Stokes I; solid black lines), total linear polarization (dashed red 
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower 
window) also shows the single pulse PPA distribution (colour scale) along with 
the average PPA (red error bars). The RVM fits to the average PPA (dashed pink 
line) is also shown in this plot. Middle panel show 
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits. Bottom panel shows the Hammer-Aitoff projection of the polarized time 
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.3}
\figsetgrptitle{PSR J0152-1637}
\figsetplot{J0152-1637_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0152-1637_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J0152-1637_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J0152-1637_602MHz_20Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars). 
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.4}
\figsetgrptitle{PSR J0304+1932}
\figsetplot{J0304+1932_317MHz_28Jun14.dat.epn2a.pdf}
\figsetplot{J0304+1932_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J0304+1932_317MHz_28Jun14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0304+1932_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0304+1932_317MHz_28Jun14.dat.epn2a.71.pdf}
\figsetplot{J0304+1932_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars). 
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits. 
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.5}
\figsetgrptitle{PSR J0452-1759}
\figsetplot{J0452-1759_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0452-1759_602MHz_09Feb14.dat.epn2a.pdf}
\figsetplot{J0452-1759_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0452-1759_602MHz_09Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0452-1759_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J0452-1759_602MHz_09Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.6}
\figsetgrptitle{PSR J0525+1115}
\figsetplot{J0525+1115_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0525+1115_602MHz_09Feb14.dat.epn2a.pdf}
\figsetplot{J0525+1115_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0525+1115_602MHz_09Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\figsetgrpstart
\figsetgrpnum{singlpol.7}
\figsetgrptitle{PSR J0528+2200}
\figsetplot{J0528+2200_317MHz_16Feb14.dat_t8.epn2a.pdf}
\figsetplot{}
\figsetplot{J0528+2200_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J0528+2200_317MHz_16Feb14.dat_t8.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.8}
\figsetgrptitle{PSR J0543+2329}
\figsetplot{J0543+2329_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0543+2329_602MHz_09Feb14.dat.epn2a.pdf}
\figsetplot{J0543+2329_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0543+2329_602MHz_09Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0543+2329_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J0543+2329_602MHz_09Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.9}
\figsetgrptitle{PSR J0614+2229}
\figsetplot{J0614+2229_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0614+2229_602MHz_09Feb14.dat.epn2a.pdf}
\figsetplot{J0614+2229_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0614+2229_602MHz_09Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0614+2229_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.10}
\figsetgrptitle{PSR J0629+2415}
\figsetplot{J0629+2415_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0629+2415_602MHz_09Feb14.dat.epn2a.pdf}
\figsetplot{J0629+2415_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0629+2415_602MHz_09Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0629+2415_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J0629+2415_602MHz_09Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.11}
\figsetgrptitle{PSR J0630-2834}
\figsetplot{J0630-2834_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J0630-2834_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J0630-2834_317MHz_28Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0630-2834_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0630-2834_317MHz_28Mar14.dat.epn2a.71.pdf}
\figsetplot{J0630-2834_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.12}
\figsetgrptitle{PSR J0659+1414}
\figsetplot{J0659+1414_317MHz_28Jun14.dat.epn2a.pdf}
\figsetplot{J0659+1414_602MHz_09Feb14.dat.epn2a.pdf}
\figsetplot{J0659+1414_317MHz_28Jun14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0659+1414_602MHz_09Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0659+1414_317MHz_28Jun14.dat.epn2a.71.pdf}
\figsetplot{J0659+1414_602MHz_09Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.13}
\figsetgrptitle{PSR J0729-1836}
\figsetplot{J0729-1836_317MHz_28Jun14.dat.epn2a.pdf}
\figsetplot{J0729-1836_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J0729-1836_317MHz_28Jun14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0729-1836_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0729-1836_317MHz_28Jun14.dat.epn2a.71.pdf}
\figsetplot{J0729-1836_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.14}
\figsetgrptitle{PSR J0738-4042}
\figsetplot{}
\figsetplot{J0738-4042_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J0738-4042_602MHz_20Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.15}
\figsetgrptitle{PSR J0742-2822}
\figsetplot{J0742-2822_317MHz_09Mar14.dat.epn2a.pdf}
\figsetplot{J0742-2822_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J0742-2822_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0742-2822_317MHz_09Mar14.dat.epn2a.71.pdf}
\figsetplot{J0742-2822_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.16}
\figsetgrptitle{PSR J0758-1528}
\figsetplot{}
\figsetplot{J0758-1528_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J0758-1528_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.17}
\figsetgrptitle{PSR J0820-1350}
\figsetplot{}
\figsetplot{J0820-1350_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J0820-1350_602MHz_20Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.18}
\figsetgrptitle{PSR J0837+0610}
\figsetplot{J0837+0610_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J0837+0610_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J0837+0610_317MHz_14Feb14.dat.epn2a.71.pdf}
\figsetplot{J0837+0610_602MHz_10Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.19}
\figsetgrptitle{PSR J0846-3533}
\figsetplot{J0846-3533_317MHz_28Jun14.dat.epn2a.pdf}
\figsetplot{J0846-3533_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{J0846-3533_317MHz_28Jun14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0846-3533_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.20}
\figsetgrptitle{PSR J0905-4536}
\figsetplot{}
\figsetplot{J0905-4536_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J0905-4536_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}}}
\figsetplot{}
\figsetplot{}
\figsetplot{}Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpnote{}
\figsetgrpend


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\figsetgrpstart
\figsetgrpnum{singlpol.21}
\figsetgrptitle{PSR J0922+0638}
\figsetplot{J0922+0638_317MHz_28Jun14.dat.epn2a.pdf}
\figsetplot{J0922+0638_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J0922+0638_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0922+0638_317MHz_28Jun14.dat.epn2a.71.pdf}
\figsetplot{J0922+0638_602MHz_20Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.22}
\figsetgrptitle{PSR J0944-1354}
\figsetplot{J0944-1354_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J0944-1354_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{J0944-1354_317MHz_28Jun14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0944-1354_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0944-1354_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.23}
\figsetgrptitle{PSR J0953+0755}
\figsetplot{J0953+0755_317MHz_14Mar14.dat.1.epn2a.pdf}
\figsetplot{J0953+0755_602MHz_07Mar14.dat.epn2a.pdf}
\figsetplot{J0953+0755_317MHz_14Mar14.dat.1.orderf.dat_chisq.pdf}
\figsetplot{J0953+0755_602MHz_07Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J0953+0755_317MHz_14Mar14.dat.1.epn2a.71.pdf}
\figsetplot{J0953+0755_602MHz_07Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.24}
\figsetgrptitle{PSR J0959-4809}
\figsetplot{}
\figsetplot{J0959-4809_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J0959-4809_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.25}
\figsetgrptitle{PSR J1034-3224}
\figsetplot{J1034-3224_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J1034-3224_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1034-3224_602MHz_10Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1034-3224_317MHz_14Feb14.dat.epn2a.71.pdf}
\figsetplot{J1034-3224_602MHz_10Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.26}
\figsetgrptitle{PSR J1041-1942}
\figsetplot{}
\figsetplot{J1041-1942_602MHz_10Aug14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1041-1942_602MHz_10Aug14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J1041-1942_602MHz_10Aug14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.27}
\figsetgrptitle{PSR J1116-4122}
\figsetplot{J1116-4122_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1116-4122_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only for 333 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.28}
\figsetgrptitle{PSR J1136+1551}
\figsetplot{J1136+1551_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J1136+1551_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{J1136+1551_317MHz_16Feb14.dat.1.orderf.dat_chisq.pdf}
\figsetplot{J1136+1551_602MHz_10Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1136+1551_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J1136+1551_602MHz_10Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.29}
\figsetgrptitle{PSR J1239+2453}
\figsetplot{J1239+2453_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J1239+2453_602MHz_26Feb14.dat.epn2a.pdf}
\figsetplot{J1239+2453_317MHz_28Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1239+2453_602MHz_26Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1239+2453_317MHz_28Mar14.dat.epn2a.71.pdf}
\figsetplot{J1239+2453_602MHz_26Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.30}
\figsetgrptitle{PSR J1321+8323}
\figsetplot{}
\figsetplot{J1321+8323_602MHz_10Aug14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1321+8323_602MHz_10Aug14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.]
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.31}
\figsetgrptitle{PSR J1328-4357}
\figsetplot{J1328-4357_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J1328-4357_602MHz_10Aug14.dat.epn2a.pdf}
\figsetplot{J1328-4357_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1328-4357_602MHz_10Aug14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.32}
\figsetgrptitle{PSR J1328-4921}
\figsetplot{J1328-4921_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J1328-4921_602MHz_05Mar14.dat.epn2a.pdf}
\figsetplot{J1328-4921_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1328-4921_602MHz_05Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1328-4921_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{}
\figsetplot{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.33}
\figsetgrptitle{PSR J1507-4352}
\figsetplot{J1507-4352_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J1507-4352_602MHz_05Mar14.dat.epn2a.pdf}
\figsetplot{J1507-4352_317MHz_14Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1507-4352_602MHz_05Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.34}
\figsetgrptitle{PSR J1527-3931}
\figsetplot{J1527-3931_317MHz_05may14.dat_t4.epn2a.pdf}
\figsetplot{J1527-3931_602MHz_26Feb14.dat_t4.epn2a.pdf}
\figsetplot{J1527-3931_317MHz_05may14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1527-3931_602MHz_26Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1527-3931_317MHz_05may14.dat_t4.epn2a.71.pdf}
\figsetplot{J1527-3931_602MHz_26Feb14.dat_t4.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.35}
\figsetgrptitle{PSR J1555-3134}
\figsetplot{J1555-3134_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J1555-3134_602MHz_26Feb14.dat.epn2a.pdf}
\figsetplot{J1555-3134_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1555-3134_602MHz_26Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.36}
\figsetgrptitle{PSR J1559-4438}
\figsetplot{J1559-4438_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J1559-4438_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J1559-4438_317MHz_14Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1559-4438_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1559-4438_317MHz_14Feb14.dat.epn2a.71.pdf}
\figsetplot{J1559-4438_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.37}
\figsetgrptitle{PSR J1603-2531}
\figsetplot{J1603-2531_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J1603-2531_602MHz_30Apr14.dat.epn2a.pdf}
\figsetplot{J1603-2531_317MHz_28Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1603-2531_602MHz_30Apr14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.38}
\figsetgrptitle{PSR J1625-4048}
\figsetplot{}
\figsetplot{J1625-4048_602MHz_07Mar14.dat_t4.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1625-4048_602MHz_07Mar14.dat_t4.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.39}
\figsetgrptitle{PSR J1645-0317}
\figsetplot{}
\figsetplot{J1645-0317_602MHz_07Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1645-0317_602MHz_07Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.40}
\figsetgrptitle{PSR J}
\figsetplot{}
\figsetplot{J1700-3312_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1700-3312_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.41}
\figsetgrptitle{PSR J1709-1640}
\figsetplot{J1709-1640_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J1709-1640_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{J1709-1640_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1709-1640_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1709-1640_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J1709-1640_602MHz_20Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.42}
\figsetgrptitle{PSR J1709-4429}
\figsetplot{}
\figsetplot{J1709-4429_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1709-4429_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.43}
\figsetgrptitle{PSR J1720-2933}
\figsetplot{J1720-2933_317MHz_14Mar14.dat.epn2a.pdf}
\figsetplot{J1720-2933_602MHz_07Mar14.dat.epn2a.pdf}
\figsetplot{J1720-2933_317MHz_14Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1720-2933_602MHz_07Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J1720-2933_602MHz_07Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.44}
\figsetgrptitle{PSR J1722-3712}
\figsetplot{J1722-3712_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J1722-3712_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{J1722-3712_317MHz_14Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1722-3712_602MHz_10Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.45}
\figsetgrptitle{PSR J1731-4744}
\figsetplot{J1731-4744_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J1731-4744_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J1731-4744_317MHz_14Feb14.dat.epn2a.71.pdf}
\figsetplot{J1731-4744_602MHz_20Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.46}
\figsetgrptitle{PSR J1733-3716}
\figsetplot{}
\figsetplot{J1733-3716_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1733-3716_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J1733-3716_602MHz_20Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.47}
\figsetgrptitle{PSR J1735-0724}
\figsetplot{J1735-0724_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1735-0724_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only for 333 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.48}
\figsetgrptitle{PSR J1740+1311}
\figsetplot{J1740+1311_317MHz_12Jul14.dat.epn2a.pdf}
\figsetplot{J1740+1311_602MHz_26Feb14.dat.epn2a.pdf}
\figsetplot{J1740+1311_317MHz_12Jul14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1740+1311_602MHz_26Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1740+1311_317MHz_12Jul14.dat.epn2a.71.pdf}
\figsetplot{J1740+1311_602MHz_26Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.49}
\figsetgrptitle{PSR J1741-0840}
\figsetplot{J1741-0840_317MHz_12Jul14.dat_t4.epn2a.pdf}
\figsetplot{J1741-0840_602MHz_23Mar14.dat_t4.epn2a.pdf}
\figsetplot{J1741-0840_317MHz_12Jul14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1741-0840_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1741-0840_317MHz_12Jul14.dat_t4.epn2a.71.pdf}
\figsetplot{J1741-0840_602MHz_23Mar14.dat_t4.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.50}
\figsetgrptitle{PSR J1741-3927}
\figsetplot{}
\figsetplot{J1741-3927_602MHz_05Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1741-3927_602MHz_05Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J1741-3927_602MHz_05Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.51}
\figsetgrptitle{PSR J1745-3040}
\figsetplot{J1745-3040_317MHz_31may14.dat.epn2a.pdf}
\figsetplot{J1745-3040_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J1745-3040_317MHz_31may14.dat.epn2a.71.pdf}
\figsetplot{J1745-3040_602MHz_10Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.52}
\figsetgrptitle{PSR J1751-4657}
\figsetplot{J1751-4657_317MHz_19Mar14.dat.epn2a.pdf}
\figsetplot{J1751-4657_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{J1751-4657_317MHz_19Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1751-4657_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1751-4657_317MHz_19Mar14.dat.epn2a.71.pdf}
\figsetplot{J1751-4657_602MHz_20Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.53}
\figsetgrptitle{PSR J}
\figsetplot{J1752-2806_317MHz_30Mar14.dat.epn2a.pdf}
\figsetplot{J1752-2806_602MHz_27Mar2014.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J1752-2806_317MHz_30Mar14.dat.epn2a.71.pdf}
\figsetplot{J1752-2806_602MHz_27Mar2014.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.54}
\figsetgrptitle{PSR J1801-0357}
\figsetplot{J1801-0357_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J1801-0357_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J1801-0357_317MHz_28Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1801-0357_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.55}
\figsetgrptitle{PSR J1801-2920}
\figsetplot{J1801-2920_317MHz_30Mar14.dat.epn2a.pdf}
\figsetplot{J1801-2920_602MHz_27Mar2014.dat.epn2a.pdf}
\figsetplot{J1801-2920_317MHz_30Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1801-2920_602MHz_27Mar2014.dat.orderf.dat_chisq.pdf}
\figsetplot{J1801-2920_317MHz_30Mar14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.56}
\figsetgrptitle{PSR J1807-0847}
\figsetplot{J1807-0847_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J1807-0847_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J1807-0847_317MHz_28Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1807-0847_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.57}
\figsetgrptitle{PSR J1808-0813}
\figsetplot{J1808-0813_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J1808-0813_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J1808-0813_317MHz_28Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1808-0813_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.58}
\figsetgrptitle{PSR J1816-2650}
\figsetplot{J1816-2650_317MHz_30Mar14.dat.epn2a.pdf}
\figsetplot{J1816-2650_602MHz_27Mar2014.dat.epn2a.pdf}
\figsetplot{J1816-2650_317MHz_30Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1816-2650_602MHz_27Mar2014.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.59}
\figsetgrptitle{PSR J1817-3618}
\figsetplot{J1817-3618_317MHz_19Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1817-3618_317MHz_19Mar14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only for 333 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.60}
\figsetgrptitle{PSR J1820-0427}
\figsetplot{J1820-0427_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J1820-0427_602MHz_27Mar2014.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1820-0427_602MHz_27Mar2014.dat.orderf.dat_chisq.pdf}
\figsetplot{J1820-0427_317MHz_28Mar14.dat.epn2a.71.pdf}
\figsetplot{J1820-0427_602MHz_27Mar2014.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.61}
\figsetgrptitle{PSR J1822-2256}
\figsetplot{J1822-2256_317MHz_31may14.dat.epn2a.pdf}
\figsetplot{J1822-2256_602MHz_27Mar2014.dat.1.epn2a.pdf}
\figsetplot{J1822-2256_317MHz_31may14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1822-2256_602MHz_27Mar2014.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J1822-2256_602MHz_27Mar2014.dat.1.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.62}
\figsetgrptitle{PSR J1823+0550}
\figsetplot{J1823+0550_317MHz_12Jul14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1823+0550_317MHz_12Jul14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only for 333 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figsetgrpstart
\figsetgrpnum{singlpol.63}
\figsetgrptitle{PSR J1823-3106}
\figsetplot{J1823-3106_317MHz_28Mar14.dat.epn2a.pdf}
\figsetplot{J1823-3106_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J1823-3106_317MHz_28Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1823-3106_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1823-3106_317MHz_28Mar14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.64}
\figsetgrptitle{PSR J1834-0426}
\figsetplot{J1834-0426_317MHz_19Mar14.dat.epn2a.pdf}
\figsetplot{J1834-0426_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{J1834-0426_317MHz_19Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1834-0426_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.65}
\figsetgrptitle{PSR J1841+0912}
\figsetplot{J1841+0912_317MHz_30Mar14.dat.epn2a.pdf}
\figsetplot{J1841+0912_602MHz_26Feb14.dat.epn2a.pdf}
\figsetplot{J1841+0912_317MHz_30Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1841+0912_602MHz_26Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.66}
\figsetgrptitle{PSR J1842-0359}
\figsetplot{}
\figsetplot{J1842-0359_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1842-0359_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel only for 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.67}
\figsetgrptitle{PSR J1900-2600}
\figsetplot{J1900-2600_317MHz_14Mar14.dat.epn2a.pdf}
\figsetplot{J1900-2600_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{J1900-2600_317MHz_14Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1900-2600_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1900-2600_317MHz_14Mar14.dat.epn2a.71.pdf}
\figsetplot{J1900-2600_602MHz_20Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.68}
\figsetgrptitle{PSR J}
\figsetplot{J1901-0906_317MHz_27jul14.dat.epn2a.pdf}
\figsetplot{J1901-0906_602MHz_07Mar14.dat.epn2a.pdf}
\figsetplot{J1901-0906_317MHz_27jul14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1901-0906_602MHz_07Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1901-0906_317MHz_27jul14.dat.epn2a.71.pdf}
\figsetplot{J1901-0906_602MHz_07Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.69}
\figsetgrptitle{PSR J1909+1102}
\figsetplot{J1909+1102_317MHz_14Mar14.dat.epn2a.pdf}
\figsetplot{J1909+1102_602MHz_26Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J1909+1102_317MHz_14Mar14.dat.epn2a.71.pdf}
\figsetplot{J1909+1102_602MHz_26Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.70}
\figsetgrptitle{PSR J1910+0358}
\figsetplot{J1910+0358_317MHz_12Jul14.dat_t4.epn2a.pdf}
\figsetplot{J1910+0358_602MHz_05Mar14.dat_t4.epn2a.pdf}
\figsetplot{J1910+0358_317MHz_12Jul14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1910+0358_602MHz_05Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.71}
\figsetgrptitle{PSR J1913-0440}
\figsetplot{J1913-0440_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J1913-0440_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J1913-0440_317MHz_14Feb14.dat.epn2a.71.pdf}
\figsetplot{J1913-0440_602MHz_10Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.72}
\figsetgrptitle{PSR J1917+1353}
\figsetplot{J1917+1353_317MHz_09Mar14.dat.epn2a.pdf}
\figsetplot{J1917+1353_602MHz_26Feb14.dat.epn2a.pdf}
\figsetplot{J1917+1353_317MHz_09Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1917+1353_602MHz_26Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.73}
\figsetgrptitle{PSR J1919+0021}
\figsetplot{J1919+0021_317MHz_21Jun14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1919+0021_317MHz_21Jun14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only for 333 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.74}
\figsetgrptitle{PSR J1919+0134}
\figsetplot{}
\figsetplot{J1919+0134_602MHz_30Apr14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J1919+0134_602MHz_30Apr14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel only for 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel only at 618 MHz  show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.75}
\figsetgrptitle{PSR J1921+2153}
\figsetplot{}
\figsetplot{J1921+2153_602MHz_30Apr14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J1921+2153_602MHz_30Apr14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel only at 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only at 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.76}
\figsetgrptitle{PSR J1932+1059}
\figsetplot{J1932+1059_317MHz_05may14.dat.1.epn2a.pdf}
\figsetplot{J1932+1059_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J1932+1059_317MHz_05may14.dat.1.epn2a.71.pdf}
\figsetplot{J1932+1059_602MHz_10Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.77}
\figsetgrptitle{PSR J1941-2602}
\figsetplot{J1941-2602_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J1941-2602_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{J1941-2602_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J1941-2602_602MHz_20Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.78}
\figsetgrptitle{PSR J1946+1805}
\figsetplot{J1946+1805_317MHz_12Jul14.dat.epn2a.pdf}
\figsetplot{J1946+1805_602MHz_30Apr14.dat.epn2a.pdf}
\figsetplot{J1946+1805_317MHz_12Jul14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1946+1805_602MHz_30Apr14.dat.orderf.dat_chisq.pdf}
\figsetplot{J1946+1805_317MHz_12Jul14.dat.epn2a.71.pdf}
\figsetplot{J1946+1805_602MHz_30Apr14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.79}
\figsetgrptitle{PSR J2006-0807}
\figsetplot{J2006-0807_317MHz_14Feb14.dat.epn2a.pdf}
\figsetplot{J2006-0807_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{J2006-0807_317MHz_14Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2006-0807_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2006-0807_317MHz_14Feb14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only for 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.80}
\figsetgrptitle{PSR J2046+1540}
\figsetplot{}
\figsetplot{J2046+1540_602MHz_20Feb14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J2046+1540_602MHz_20Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{}
\figsetgrpnote{Top panel only at 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Bottom panel only at 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.81}
\figsetgrptitle{PSR J2046-0421}
\figsetplot{J2046-0421_317MHz_16Feb14.dat.epn2a.pdf}
\figsetplot{J2046-0421_602MHz_10Feb14.dat.epn2a.pdf}
\figsetplot{J2046-0421_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2046-0421_602MHz_10Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2046-0421_317MHz_16Feb14.dat.epn2a.71.pdf}
\figsetplot{J2046-0421_602MHz_10Feb14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.82}
\figsetgrptitle{PSR J2048-1616}
\figsetplot{J2048-1616_317MHz_19Mar14.dat.epn2a.pdf}
\figsetplot{J2048-1616_602MHz_20Mar14.dat.epn2a.pdf}
\figsetplot{J2048-1616_317MHz_19Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2048-1616_602MHz_20Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2048-1616_317MHz_19Mar14.dat.epn2a.71.pdf}
\figsetplot{J2048-1616_602MHz_20Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.83}
\figsetgrptitle{PSR J2144-3933}
\figsetplot{J2144-3933_317MHz_16Feb14.dat_t8.epn2a.pdf}
\figsetplot{}
\figsetplot{J2144-3933_317MHz_16Feb14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J2144-3933_317MH only for 333 MHzz_16Feb14.dat_t8.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only at 618 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only at 618 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only at 618 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.84}
\figsetgrptitle{PSR J2305+3100}
\figsetplot{J2305+3100_317MHz_27jul14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{J2305+3100_317MHz_27jul14.dat.orderf.dat_chisq.pdf}
\figsetplot{}
\figsetplot{J2305+3100_317MHz_27jul14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only at 333 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel only at 333 MHz show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel only at 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.85}
\figsetgrptitle{PSR J2313+4253}
\figsetplot{J2313+4253_317MHz_27jul14.dat.epn2a.pdf}
\figsetplot{}
\figsetplot{}
\figsetplot{}
\figsetplot{J2313+4253_317MHz_27jul14.dat.epn2a.71.pdf}
\figsetplot{}
\figsetgrpnote{Top panel only at 333 MHz (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
Bottom panel only at 333 MHz shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.86}
\figsetgrptitle{PSR J2317+2149}
\figsetplot{J2317+2149_317MHz_21Jun14.dat.epn2a.pdf}
\figsetplot{J2317+2149_602MHz_27Mar2014.dat.epn2a.pdf}
\figsetplot{J2317+2149_317MHz_21Jun14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2317+2149_602MHz_27Mar2014.dat.orderf.dat_chisq.pdf}
\figsetplot{J2317+2149_317MHz_21Jun14.dat.epn2a.71.pdf}
\figsetplot{J2317+2149_602MHz_27Mar2014.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\figsetgrpstart
\figsetgrpnum{singlpol.87}
\figsetgrptitle{PSR J2330-2005}
\figsetplot{J2330-2005_317MHz_05may14.dat.1.epn2a.pdf}
\figsetplot{J2330-2005_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J2330-2005_317MHz_05may14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2330-2005_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2330-2005_317MHz_05may14.dat.1.epn2a.71.pdf}
\figsetplot{J2330-2005_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetgrpstart
\figsetgrpnum{singlpol.88}
\figsetgrptitle{PSR J2346-0609}
\figsetplot{J2346-0609_317MHz_21Jun14.dat.epn2a.pdf}
\figsetplot{J2346-0609_602MHz_23Mar14.dat.epn2a.pdf}
\figsetplot{J2346-0609_317MHz_21Jun14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2346-0609_602MHz_23Mar14.dat.orderf.dat_chisq.pdf}
\figsetplot{J2346-0609_317MHz_21Jun14.dat.epn2a.71.pdf}
\figsetplot{J2346-0609_602MHz_23Mar14.dat.epn2a.71.pdf}
\figsetgrpnote{Top panel (upper window) shows the average profile with total
intensity (Stokes I; solid black lines), total linear polarization (dashed red
line) and circular polarization (Stokes V; dotted blue line). Top panel (lower
window) also shows the single pulse PPA distribution (colour scale) along with
the average PPA (red error bars).
The RVM fits to the average PPA (dashed pink
line) is also shown in this plot. Middle panel show
the $\chi^2$ contours for the parameters $\alpha$ and $\beta$ obtained from RVM
fits.
Bottom panel shows the Hammer-Aitoff projection of the polarized time
samples with the colour scheme representing the fractional polarization level.}
\figsetgrpend



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figsetend

